Revisiting Early-Learning Regularization When Federated Learning Meets Noisy Labels

In the evolving landscape of federated learning (FL), addressing label noise presents unique challenges due to the decentralized and diverse nature of data collection across clients. Traditional centralized learning approaches to mitigate label noise are constrained in FL by privacy concerns and the heterogeneity of client data. This paper revisits early-learning regularization, introducing an innovative strategy, Federated Label-mixture Regularization (FLR). FLR adeptly adapts to FL's complexities by generating new pseudo labels, blending local and global model predictions. This method not only enhances the accuracy of the global model in both i.i.d. and non-i.i.d. settings but also effectively counters the memorization of noisy labels. Demonstrating compatibility with existing label noise and FL techniques, FLR paves the way for improved generalization in FL environments fraught with label inaccuracies.

==> tables/cifar10.tex <==
\begin{table*}[t]
\caption[CIFAR-10 with IID setting (1)]{Average and standard deviation of the best test accuracy of 5 trials for each method, on CIFAR-10 with i.i.d. setting and different noise levels. The highest accuracy for each noise level is boldfaced. `Centralized' refers to the server conducting SGD training with all the data corrupted by the same scheme in the federated environment.}
\vspace{-5pt}
\begin{center}
\resizebox{\textwidth}{!}{\begin{tabular}{ll|c|ccc|ccc|ccc}
	\toprule
	\multirow{4}{*}{Setting} & \multirow{4}{*}{Method} & Clean & \multicolumn{6}{c|}{Symmetric} & \multicolumn{3}{c}{Asymmetric} \\
	\cmidrule{3-12}
	& & $\tau=0.0$ & \multicolumn{3}{c|}{$\tau=0.0$} & \multicolumn{3}{c|}{$\tau=0.5$} & \multicolumn{3}{c}{$\tau=0.4$} \\
	\cmidrule{3-12}
	& & $\rho=0.0$ & $\rho=0.4$ & $\rho=0.6$ & $\rho=0.8$ & $\rho=0.4$ & $\rho=0.6$ & $\rho=0.8$ & $\rho=0.4$ & $\rho=0.6$ & $\rho=0.8$ \\
	\midrule
	Centralized
		& CE & 92.65$\pm$0.12 & 84.37$\pm$0.45 & 85.69$\pm$0.68 & 82.12$\pm$0.43 & 84.46$\pm$0.30 & 80.93$\pm$0.40 & 75.35$\pm$1.07 & 88.59$\pm$0.20 & 86.93$\pm$0.32 & 85.07$\pm$0.62 \\
		& GCE & 91.67$\pm$0.12 & 90.19$\pm$0.15 & 89.35$\pm$0.47 & 87.99$\pm$0.37 &  89.28$\pm$0.26 & 87.28$\pm$0.28 & 83.94$\pm$0.46 & 90.20$\pm$0.14 & 88.74$\pm$0.20 & 86.27$\pm$0.33  \\
		& Mixup & \textbf{93.57$\pm$0.09} & 89.34$\pm$0.58 & 87.35$\pm$0.41 & 84.98$\pm$0.73 & 87.63$\pm$0.41 & 83.91$\pm$0.28 & 79.14$\pm$0.57 & 90.93$\pm$0.30 & 89.45$\pm$0.51 & 87.25$\pm$0.34 \\
		& Co-teaching & 92.71$\pm$0.04 & 86.62$\pm$0.82 & 84.54$\pm$0.72 & 82.00$\pm$0.69 & 84.38$\pm$0.50 & 80.46$\pm$0.49 & 75.26$\pm$1.01 &  \textbf{91.20$\pm$0.15} & \textbf{89.95$\pm$0.15} & \textbf{88.53$\pm$0.27} \\
		& DivideMix & 86.84$\pm$0.49 & 88.33$\pm$0.75 & 90.05$\pm$0.42 & \textbf{90.52$\pm$0.34} & 90.45$\pm$0.27 & \textbf{90.63$\pm$0.31} & \textbf{89.38$\pm$0.21} & 83.26$\pm$0.62 & 81.57$\pm$0.34 & 80.96$\pm$0.83  \\
            & ELR & 93.06$\pm$0.05 & \textbf{91.69$\pm$0.25} & \textbf{90.95$\pm$0.45} & 89.61$\pm$0.30 & \textbf{90.81$\pm$0.28} & 88.96$\pm$0.15 & 85.64$\pm$0.34 & 90.05$\pm$0.17 & 88.87$\pm$0.19 & 86.66$\pm$0.38  \\
	\specialrule{.1em}{.05em}{.05em}
	FedAvg
		& CE & 90.42$\pm$0.34 & 81.30$\pm$1.06 & 74.58$\pm$1.00 & 67.76$\pm$1.14 & 75.97$\pm$0.43 & 66.99$\pm$0.98 & 55.67$\pm$1.05 & 87.63$\pm$0.20 & 85.90$\pm$0.25 & 83.13$\pm$0.35 \\
		& GCE & 87.89$\pm$0.28 & 85.96$\pm$0.54 & 84.94$\pm$0.54 & 82.80$\pm$0.69 & 84.82$\pm$0.42 & 81.66$\pm$0.87 & {74.15$\pm$0.62} & 87.97$\pm$0.27 & 86.95$\pm$0.24 & 85.13$\pm$0.38  \\
		& Mixup & 90.43$\pm$0.15 & 86.32$\pm$0.56 & 83.11$\pm$0.70 & 78.22$\pm$0.52 & 84.26$\pm$0.29 & 77.16$\pm$0.21 & 65.47$\pm$0.91 & 88.64$\pm$0.25 & 86.87$\pm$0.22 & 83.94$\pm$0.64  \\
		& Co-teaching & 90.42$\pm$0.23 & 82.27$\pm$0.59 & 76.11$\pm$1.08 & 70.37$\pm$0.76 & 76.30$\pm$0.64 & 67.73$\pm$0.98 & 57.98$\pm$0.78 & 86.79$\pm$0.17 & 84.94$\pm$0.12 & 82.54$\pm$0.41  \\
		& DivideMix & 66.91$\pm$0.65 & 68.78$\pm$0.31 & 70.24$\pm$0.78 & 72.32$\pm$0.64 & 68.61$\pm$1.14 & 69.35$\pm$0.72 & 68.40$\pm$2.79 & 66.40$\pm$0.68 & 65.97$\pm$1.18 & 63.54$\pm$0.59  \\
		& ELR & {91.65$\pm$0.11} & 89.28$\pm$0.36 & 87.49$\pm$0.45 & 84.09$\pm$0.78 & 87.67$\pm$0.38 & 82.29$\pm$0.15 & 70.86$\pm$1.31 & 90.76$\pm$0.16 & 89.78$\pm$0.12 & 87.44$\pm$0.33  \\
		 & ER & 91.42$\pm$0.03 & 88.58$\pm$0.22 & 86.45$\pm$0.45 & 83.12$\pm$0.88 & 86.64$\pm$0.23 & 80.51$\pm$0.61 & 70.02$\pm$1.63 & 89.90$\pm$0.22 & 88.73$\pm$0.24 & 86.35$\pm$0.42 \\
		 & SLR & 91.32$\pm$0.10 & {89.43$\pm$0.16} & {87.99$\pm$0.38} & {85.63$\pm$0.48} & {88.26$\pm$0.16} & {84.36$\pm$0.24} & 73.28$\pm$2.22 & {90.78$\pm$0.12} & {90.22$\pm$0.11} & {89.64$\pm$0.19} \\
           \rowcolor{gray!20}\cellcolor{white}  &  {FLR} & \textbf{91.88$\pm$0.17} & \textbf{89.90$\pm$0.13} & \textbf{88.07$\pm$0.18} & \textbf{86.82$\pm$0.71} & \textbf{88.71$\pm$0.14} & \textbf{84.78$\pm$0.20} & \textbf{75.22$\pm$1.93} & \textbf{90.94$\pm$0.08} & \textbf{90.55$\pm$0.14} & \textbf{89.93$\pm$0.21} \\
	\midrule
	FedProx
	    & CE & 89.83$\pm$0.11 & 80.80$\pm$0.70 & 74.44$\pm$1.41 & 67.36$\pm$0.70 & 75.22$\pm$2.12 & 66.67$\pm$2.04 & 53.10$\pm$0.85 & 86.95$\pm$0.44 & 85.08$\pm$0.67 & 81.84$\pm$0.59 \\
	\specialrule{.1em}{.05em}{.05em}
	FedCorr
		& CE & 92.40$\pm$0.13 & 89.32$\pm$0.50 & 86.77$\pm$0.69 & 81.77$\pm$0.87 & 88.40$\pm$0.31 & 82.29$\pm$0.60 & 68.33$\pm$1.66 & 89.99$\pm$0.13 & 88.49$\pm$0.32 & 86.12$\pm$0.73 \\
		& Mixup & {93.49$\pm$0.17} & 91.70$\pm$0.16 & 90.37$\pm$0.41 & 87.52$\pm$0.62 & 91.06$\pm$0.07 & 88.88$\pm$0.43 & 83.59$\pm$1.65 & 91.45$\pm$0.19  & 89.95$\pm$0.33 & 87.61$\pm$0.30 \\
            & ELR & {92.88$\pm$0.08} & 92.72$\pm$0.14 & 90.92$\pm$0.24 & 90.05$\pm$0.22 & 92.12$\pm$0.15 & 90.93$\pm$0.48 & 86.74$\pm$0.83 & 92.31$\pm$0.17  & {90.98$\pm$0.26} & 90.82$\pm$0.23 \\
         & ER & 93.33$\pm$0.14 & 92.31$\pm$0.19 & 91.11$\pm$0.13 & 89.87$\pm$0.29 & 91.94$\pm$0.56 & 90.15$\pm$0.33 & 86.99$\pm$0.90 & 92.01$\pm$0.19 & 91.12$\pm$0.37 & 90.06$\pm$0.22  \\
         & SLR & 93.40$\pm$0.12 & {92.76$\pm$0.14} & {91.87$\pm$0.33} & {90.79$\pm$0.31} & 92.40$\pm$0.20 & {91.11$\pm$0.18} & 88.68$\pm$0.77 & {92.43$\pm$0.10} & {91.81$\pm$0.11} & {91.06$\pm$0.25}  \\
		 \rowcolor{gray!20}\cellcolor{white}  & {FLR} & \textbf{93.51$\pm$0.12} & \textbf{92.98$\pm$0.10} & \textbf{91.96$\pm$0.27} & \textbf{91.33$\pm$0.36} & \textbf{92.63$\pm$0.18} & \textbf{91.34$\pm$0.13} & \textbf{88.81$\pm$0.70} & \textbf{92.83$\pm$0.09} & \textbf{91.90$\pm$0.13} & \textbf{91.11$\pm$0.16}  \\
	\bottomrule
\end{tabular}}
\end{center}
\label{tab:cifar10}
\end{table*}


==> tables/cifar100_di10_0.3.tex <==
\begin{table*}[h]\small
\caption[CIFAR-100 with non-i.i.d. setting of $(p,\alpha)=(0.3,10)$]{Average and standard deviation of the best test accuracy of 5 trials for each method, on CIFAR-100 with non-i.i.d. setting of $(p,\alpha)=(0.3,10)$ and different noise levels. The highest accuracy for each noise level is boldfaced.}
\begin{center}
\begin{tabular}{ll|c|cc|cc}
	\toprule
	\multirow{4}{*}{Algorithm} & \multirow{4}{*}{Method} & Clean & \multicolumn{2}{c|}{Symmetric} & \multicolumn{2}{c}{Asymmetric} \\
	\cmidrule{3-7}
	& & $\gamma=0.0$ & \multicolumn{2}{c|}{$\tau=0.0$} & \multicolumn{2}{c}{$\tau=0.4$} \\
	\cmidrule{3-7}
	& & $\rho=0.0$ & $\rho=0.6$ & $\rho=0.8$ & $\rho=0.6$ & $\rho=0.8$ \\
	\midrule
	FedAvg
		& CE & 62.50$\pm$0.58 & 37.23$\pm$1.37 & 31.42$\pm$2.69 & 47.95$\pm$0.62 & 42.25$\pm$1.18 \\
		& Mixup & 57.64$\pm$0.48 & 39.31$\pm$1.45 & 35.32$\pm$2.43 & 45.87$\pm$1.05 & 40.53$\pm$1.03 \\
            & ELR & \textbf{67.08$\pm$0.38} & \textbf{48.49$\pm$1.68} & 40.81$\pm$2.70 & 53.74$\pm$0.64 & 47.27$\pm$0.97 \\
		& SLR & 64.89$\pm$0.44 & 46.83$\pm$1.98 & 39.07$\pm$2.58 & {55.14$\pm$0.27} & {47.64$\pm$0.88} \\
            \rowcolor{gray!20}\cellcolor{white} & FLR & {65.12$\pm$0.36} & 47.15$\pm$1.88 & 39.24$\pm$2.11 & \textbf{55.90$\pm$0.21} & \textbf{48.23$\pm$0.79} \\
		\rowcolor{gray!20}\cellcolor{white} & FLR$^+$ & 62.31$\pm$0.38 & 47.00$\pm$1.64 & \textbf{41.66$\pm$2.75} & 52.54$\pm$0.78 & 47.33$\pm$1.19 \\
	\midrule
	FedProx
		& CE & 60.52$\pm$0.70 & 34.87$\pm$1.63 & 29.96$\pm$2.61 & 45.47$\pm$0.81 & 39.28$\pm$1.93 \\
	\specialrule{.1em}{.05em}{.05em}
	FedCorr
		& Mixup & 63.43$\pm$0.55 & 50.84$\pm$1.13 & 46.26$\pm$1.28 & 53.39$\pm$0.67 & 47.06$\pm$0.97 \\
		& SLR & \textbf{66.92$\pm$0.39} & {55.01$\pm$1.04} & {50.19$\pm$2.71} & {56.61$\pm$1.69} & \textbf{49.15$\pm$1.21} \\
            \rowcolor{gray!20}\cellcolor{white} & FLR & {66.73$\pm$0.25} & \textbf{55.33$\pm$1.17} & \textbf{50.49$\pm$2.30} & \textbf{56.84$\pm$1.87} & {48.79$\pm$1.81} \\
	\midrule
	\bottomrule
\end{tabular}
\end{center}
\label{tab:cifar100_DI10(0.3)}
\end{table*}


==> tables/cifar100_di10_0.7.tex <==
\begin{table*}[h]\small
\caption[CIFAR-100 with non-i.i.d. setting of $(p,\alpha)=(0.7,10)$]{Average and standard deviation of the best test accuracy of 5 trials for each method, on CIFAR-100 with non-i.i.d. setting of $(p,\alpha)=(0.7,10)$ and different noise levels. The highest accuracy for each noise level is boldfaced.}
\begin{center}
\begin{tabular}{ll|c|cc|cc}
	\toprule
	\multirow{4}{*}{Algorithm} & \multirow{4}{*}{Method} & Clean & \multicolumn{2}{c|}{Symmetric} & \multicolumn{2}{c}{Asymmetric} \\
	\cmidrule{3-7}
	& & $\gamma=0.0$ & \multicolumn{2}{c|}{$\tau=0.0$} & \multicolumn{2}{c}{$\tau=0.4$} \\
	\cmidrule{3-7}
	& & $\rho=0.0$ & $\rho=0.6$ & $\rho=0.8$ & $\rho=0.6$ & $\rho=0.8$ \\
	\midrule
	FedAvg
		& CE & 64.75$\pm$0.49 & 43.24$\pm$1.68 & 36.47$\pm$2.33 & 52.90$\pm$0.74 & 47.88$\pm$0.77 \\
		& Mixup & 65.59$\pm$0.51 & 50.91$\pm$1.59 & 45.84$\pm$1.11 & 57.44$\pm$0.42 & 52.67$\pm$0.81 \\
		& ELR & \textbf{69.76$\pm$0.26} & 51.76$\pm$2.02 & 43.95$\pm$2.96 & 57.80$\pm$0.65 & 52.54$\pm$0.78 \\
		 & SLR & 69.01$\pm$0.25 & 52.03$\pm$2.18 & 45.13$\pm$2.23 & 60.84$\pm$1.19 & 55.00$\pm$1.24 \\
            \rowcolor{gray!20}\cellcolor{white} & FLR & 69.31$\pm$0.13 & 53.21$\pm$1.87 & 46.13$\pm$2.18 & 61.31$\pm$0.79 & 55.77$\pm$1.02 \\
		\rowcolor{gray!20}\cellcolor{white} & FLR$^+$ & 69.71$\pm$0.25 & \textbf{58.33$\pm$1.20} & \textbf{53.04$\pm$1.96} & \textbf{64.43$\pm$0.35} & \textbf{61.09$\pm$0.59} \\
	\midrule
	FedProx
		& CE & 62.72$\pm$0.61 & 39.83$\pm$2.05 & 33.46$\pm$2.14 & 49.58$\pm$0.46 & 43.51$\pm$0.67 \\
	\specialrule{.1em}{.05em}{.05em}
	FedCorr
		& Mixup & 71.27$\pm$0.27 & 62.19$\pm$0.85 & 57.85$\pm$0.85 & 65.46$\pm$0.29 & 60.66$\pm$0.56 \\
		 & SLR & {72.90$\pm$0.26} & {66.41$\pm$0.58} & {62.74$\pm$0.98} & {67.34$\pm$0.36} & \textbf{64.67$\pm$0.15} \\
            \rowcolor{gray!20}\cellcolor{white} & FLR & \textbf{73.16$\pm$0.27} & \textbf{67.03$\pm$0.19} & \textbf{63.46$\pm$0.87} & \textbf{67.96$\pm$0.41} & {64.57$\pm$0.09} \\
	\midrule
	\bottomrule
\end{tabular}
\end{center}
\label{tab:cifar100_DI10(0.7)}
\end{table*}


==> tables/cifar10_di10_0.3.tex <==
\begin{table}[t]
\caption[CIFAR-10 with non-IID setting of $(p,\alpha)=(0.3,10)$]{Average and standard deviation of the best test accuracy of 5 trials for each method, on CIFAR-10 with non-IID setting of $(p,\alpha)=(0.3,10)$ and different noise levels. The highest accuracy for each noise level is boldfaced.}
\addtolength{\tabcolsep}{-4pt}\tiny
\vspace{-5pt}
\begin{center}
\begin{tabular}{ll|c|cc|cc}
	\toprule
	\multirow{4}{*}{Algorithm} & \multirow{4}{*}{Method} & Clean & \multicolumn{2}{c|}{Symmetric} & \multicolumn{2}{c}{Asymmetric} \\
	\cmidrule{3-7}
	& & $\gamma=0.0$ & \multicolumn{2}{c|}{$\tau=0.0$} & \multicolumn{2}{c}{$\tau=0.4$} \\
	\cmidrule{3-7}
	& & $\rho=0.0$ & $\rho=0.6$ & $\rho=0.8$ & $\rho=0.6$ & $\rho=0.8$ \\
	\midrule
	FedAvg
		& CE & \textbf{85.74$\pm$0.77} & 64.75$\pm$3.50 & 52.77$\pm$3.89 & 78.21$\pm$1.20 & 73.83$\pm$2.21 \\
		& GCE & 82.95$\pm$1.14 & 78.94$\pm$1.66 & 75.34$\pm$1.81 & 77.36$\pm$1.64 & 70.51$\pm$1.71 \\
		& Mixup & 82.16$\pm$1.28 & 70.94$\pm$3.20 & 63.05$\pm$3.51 & 74.25$\pm$1.43 & 70.26$\pm$1.84 \\
		& Co-teaching & 85.28$\pm$0.89 & 68.90$\pm$2.75 & 60.39$\pm$2.71 & 78.85$\pm$0.60 & 75.70$\pm$1.61 \\
		& ELR & 84.20$\pm$1.90 & \textbf{80.61$\pm$2.01} & \textbf{78.37$\pm$1.60} & \textbf{84.31$\pm$0.56} & \textbf{80.90$\pm$2.25} \\
		\rowcolor{gray!20} & leLR & 84.24$\pm$1.26 & 79.21$\pm$2.01 & 74.29$\pm$2.08 & 79.68$\pm$1.46 & 74.92$\pm$1.89 \\
		\rowcolor{gray!20} & FLR & 85.08$\pm$0.54 & 77.89$\pm$1.68 & 70.08$\pm$4.09 & 77.70$\pm$1.40 & 71.28$\pm$1.06 \\
	\midrule
	FedProx
	    & CE & 84.83$\pm$0.83 & 64.19$\pm$4.63 & 52.51$\pm$5.54 & 77.46$\pm$2.23 & 72.89$\pm$1.68 \\
	\specialrule{.1em}{.05em}{.05em}
	FedCorr
	    & Mixup & 79.30$\pm$2.46 & 70.72$\pm$5.10 & 62.48$\pm$4.43 & 75.45$\pm$1.93 & 70.90$\pm$2.57 \\
		\rowcolor{gray!20} & FLR & \textbf{80.49$\pm$1.24} & \textbf{75.45$\pm$2.58} & \textbf{64.10$\pm$3.41} & \textbf{77.44$\pm$2.10} & \textbf{71.65$\pm$2.70} \\
	\midrule
	\bottomrule
\end{tabular}
\end{center}
\label{tab:cifar10_DI10(0.3)}
\end{table}


==> tables/cifar10_di10_0.7.tex <==
\begin{table}[t]
\caption[CIFAR-10 with non-IID setting of $(p,\alpha)=(0.7,10)$]{Average and standard deviation of the best test accuracy of 5 trials for each method, on CIFAR-10 with non-IID setting of $(p,\alpha)=(0.7,10)$ and different noise levels. The highest accuracy for each noise level is boldfaced.}
\begin{center}
\addtolength{\tabcolsep}{-4pt}\tiny
\vspace{-5pt}
\begin{tabular}{ll|c|cc|cc}
	\toprule
	\multirow{4}{*}{Algorithm} & \multirow{4}{*}{Method} & Clean & \multicolumn{2}{c|}{Symmetric} & \multicolumn{2}{c}{Asymmetric} \\
	\cmidrule{3-7}
	& & $\gamma=0.0$ & \multicolumn{2}{c|}{$\tau=0.0$} & \multicolumn{2}{c}{$\tau=0.4$} \\
	\cmidrule{3-7}
	& & $\rho=0.0$ & $\rho=0.6$ & $\rho=0.8$ & $\rho=0.6$ & $\rho=0.8$ \\
	\midrule
	FedAvg
		& CE & 89.74$\pm$0.23 & 76.19$\pm$2.86 & 67.23$\pm$1.90 & 85.34$\pm$0.76 & 82.32$\pm$0.58 \\
		& GCE & 87.05$\pm$0.24 & 84.07$\pm$0.78 & 82.05$\pm$1.35 & 84.24$\pm$0.51 & 81.64$\pm$1.12 \\
		& Mixup & 88.76$\pm$0.39 & 82.68$\pm$0.86 & 78.45$\pm$1.34 & 85.28$\pm$0.57 & 81.60$\pm$1.51 \\
		& Co-teaching & 89.61$\pm$0.13 & 78.08$\pm$2.24 & 71.34$\pm$1.12 & 83.89$\pm$0.29 & 80.97$\pm$0.95 \\
		& ELR & 90.05$\pm$0.30 & 86.27$\pm$0.98 & 83.37$\pm$1.27 & \textbf{88.61$\pm$0.22} & \textbf{86.42$\pm$1.14} \\
		\rowcolor{gray!20} & leLR & \textbf{90.22$\pm$0.32} & 85.99$\pm$0.68 & 82.38$\pm$1.51 & 86.98$\pm$0.65 & 84.12$\pm$0.93 \\
		\rowcolor{gray!20} & FLR & 89.84$\pm$0.18 & \textbf{86.79$\pm$0.88} & \textbf{84.59$\pm$1.29} & 87.10$\pm$2.18 & 82.90$\pm$1.30 \\
	\midrule
	FedProx
	    & CE & 88.88$\pm$0.23 & 74.69$\pm$2.84 & 65.46$\pm$1.54 & 83.84$\pm$0.83 & 81.05$\pm$0.84 \\
	\specialrule{.1em}{.05em}{.05em}
	FedCorr
	    & Mixup & \textbf{91.05$\pm$0.74} & 87.26$\pm$0.48 & 83.39$\pm$0.90 & 87.05$\pm$0.64 & 83.44$\pm$0.57 \\
		\rowcolor{gray!20} & FLR & 89.86$\pm$1.45 & \textbf{89.06$\pm$0.41} & \textbf{87.13$\pm$0.79} & \textbf{89.40$\pm$0.99} & \textbf{87.80$\pm$1.47} \\
	\midrule
	\bottomrule
\end{tabular}
\end{center}
\label{tab:cifar10_DI10(0.7)}
\end{table}


==> tables/cifar10_di10_1.0.tex <==
\begin{table}[t]
\caption[CIFAR-10 with non-i.i.d. setting of $(p,\alpha_{Dir})=(1.0,10)$]{Average and standard deviation of the best test accuracy of 5 trials for each method, on CIFAR-10 with non-i.i.d. setting of $(p,\alpha_{Dir})=(1.0,10)$ and different noise levels.}
\tiny\addtolength{\tabcolsep}{-4pt}
\vspace{-5pt}
\begin{center}
\begin{tabular}{ll|c|cc|cc}
	\toprule
	\multirow{4}{*}{Algorithm} & \multirow{4}{*}{Method} & Clean & \multicolumn{2}{c|}{Symmetric} & \multicolumn{2}{c}{Asymmetric} \\
	\cmidrule{3-7}
	& & $\gamma=0.0$ & \multicolumn{2}{c|}{$\tau=0.0$} & \multicolumn{2}{c}{$\tau=0.4$} \\
	\cmidrule{3-7}
	& & $\rho=0.0$ & $\rho=0.6$ & $\rho=0.8$ & $\rho=0.6$ & $\rho=0.8$ \\
	\midrule
	FedAvg
		& CE & 90.28$\pm$0.13 & 78.34$\pm$1.61 & 70.17$\pm$0.87 & 86.40$\pm$0.45 & 83.64$\pm$0.30 \\		
		& GCE & 87.35$\pm$0.34 & 84.58$\pm$0.67 & 82.65$\pm$0.61 & 84.82$\pm$0.38 & 82.58$\pm$0.73 \\
		& Mixup & 90.21$\pm$0.14 & 85.03$\pm$0.53 & 80.81$\pm$1.20 & 87.25$\pm$0.40 & 84.30$\pm$0.38 \\
		& Co-teaching & 90.21$\pm$0.24 & 79.81$\pm$1.01 & 72.42$\pm$1.09 & 84.21$\pm$0.52 & 81.46$\pm$0.72 \\
  		& ELR & 90.77$\pm$0.27 & 87.10$\pm$0.57 & 84.39$\pm$0.65 & \textbf{89.53$\pm$0.27} & 87.09$\pm$0.27 \\
		\rowcolor{gray!20} & LELR & \textbf{90.92$\pm$0.28} & 86.96$\pm$0.36 & 84.36$\pm$0.57 & 88.33$\pm$0.11 & 85.88$\pm$0.44 \\
		\rowcolor{gray!20} & SLR & 90.43$\pm$0.25 & \textbf{87.55$\pm$0.41} & \textbf{85.38$\pm$0.62} & 89.10$\pm$0.31 & \textbf{87.18$\pm$1.70} \\
            \rowcolor{gray!20} & FLR & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx \\
	\midrule
	FedProx
	    & CE & 89.64$\pm$0.27 & 77.65$\pm$1.79 & 68.87$\pm$0.99 & 85.39$\pm$0.72 & 82.28$\pm$0.67 \\
	\specialrule{.1em}{.05em}{.05em}
	FedCorr
		& Mixup & 92.74$\pm$0.27 & 89.50$\pm$0.50 & 86.50$\pm$0.20 & 89.57$\pm$0.51 & 87.08$\pm$0.60 \\
            & ELR & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx \\
            \rowcolor{gray!20} & LELR & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx \\
            \rowcolor{gray!20} & SLR & \textbf{92.79$\pm$0.30} & \textbf{91.19$\pm$0.56} & \textbf{89.84$\pm$0.27} & \textbf{91.37$\pm$0.21} & \textbf{90.63$\pm$0.20} \\
		\rowcolor{gray!20} & FLR & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx \\
	\bottomrule
\end{tabular}
\end{center}
\label{tab:cifar10_DI10(1.0)}
\vspace{-5pt}
\end{table}


==> tables/cifar10_di1_1.0.tex <==
\begin{table}[t]
\caption[CIFAR-10 with non-IID setting of $(p,\alpha)=(1.0,1)$]{Average and standard deviation of the best test accuracy of 5 trials for each method, on CIFAR-10 with non-i.i.d. setting of $(p,\alpha_{Dir})=(1.0,1)$ and different noise levels.}
\addtolength{\tabcolsep}{-4pt}\tiny
\vspace{-5pt}
\begin{center}
\begin{tabular}{ll|c|cc|cc}
	\toprule
	\multirow{4}{*}{Algorithm} & \multirow{4}{*}{Method} & Clean & \multicolumn{2}{c|}{Symmetric} & \multicolumn{2}{c}{Asymmetric} \\
	\cmidrule{3-7}
	& & $\gamma=0.0$ & \multicolumn{2}{c|}{$\tau=0.0$} & \multicolumn{2}{c}{$\tau=0.4$} \\
	\cmidrule{3-7}
	& & $\rho=0.0$ & $\rho=0.6$ & $\rho=0.8$ & $\rho=0.6$ & $\rho=0.8$ \\
	\midrule
	FedAvg
		& CE & 89.58$\pm$0.26 & 75.62$\pm$2.08 & 66.54$\pm$0.98 & 85.44$\pm$0.29 & 82.78$\pm$0.39 \\
		& GCE & 86.91$\pm$0.40 & 84.24$\pm$0.77 & 81.80$\pm$1.03 & 84.49$\pm$0.29 & 82.01$\pm$0.66 \\
		& Mixup & 89.18$\pm$0.34 & 83.18$\pm$1.15 & 78.00$\pm$0.64 & 85.78$\pm$0.55 & 83.25$\pm$0.85 \\
		& Co-teaching & 89.67$\pm$0.26 & 77.09$\pm$1.75 & 69.48$\pm$0.83 & 83.70$\pm$0.32 & 80.75$\pm$0.43 \\
  		& ELR & 90.17$\pm$0.39 & 86.13$\pm$0.61 & 83.43$\pm$0.81 & 88.51$\pm$0.29 & \textbf{86.65$\pm$0.43} \\
            \rowcolor{gray!20} & LELR & \textbf{90.26$\pm$0.25} & 85.34$\pm$0.86 & 81.76$\pm$0.71 & 87.28$\pm$0.24 & 85.06$\pm$0.52 \\
		\rowcolor{gray!20} & SLR & 89.94$\pm$0.28 & \textbf{86.90$\pm$0.57} & \textbf{84.09$\pm$0.67} & \textbf{88.61$\pm$0.27} & 86.16$\pm$0.88 \\
            \rowcolor{gray!20} & FLR & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx \\
	\midrule
	FedProx
	    & CE & 89.13$\pm$0.39 & 75.03$\pm$1.15 & 66.52$\pm$0.90 & 84.59$\pm$0.68 & 81.17$\pm$0.41 \\
	\specialrule{.1em}{.05em}{.05em}
	FedCorr
		& Mixup & \textbf{91.71$\pm$0.26} & 86.51$\pm$1.03 & 83.84$\pm$0.79 & 88.24$\pm$0.41 & 85.49$\pm$0.49 \\
            & ELR & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx \\
            \rowcolor{gray!20} & LELR & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx \\
		\rowcolor{gray!20} & SLR & 91.23$\pm$0.45 & \textbf{88.92$\pm$0.48} & \textbf{87.55$\pm$0.57} & \textbf{89.88$\pm$0.45} & \textbf{88.72$\pm$0.93} \\
            \rowcolor{gray!20} & FLR & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx & xx.xx$\pm$x.xx \\
	\bottomrule
\end{tabular}
\end{center}
\label{tab:cifar10_DI1(1.0)}
\end{table}


==> tables/cifar10n.tex <==
\begin{table*}[t]
\caption{Test accuracies for each method, evaluated on CIFAR10N dataset in federated scenarios with uniformly random distributed settings. }
\vspace{-5pt}
\begin{center}\scriptsize
\begin{tabular}{ccccccc|c|cc}
	\toprule
	Type  & CE & Mixup & ELR & ER & SLR & \cellcolor{gray!20}FLR & FedProx & FedCorr & \cellcolor{gray!20}FedCorr+FLR\\
	\midrule
	Aggregate & 80.09 & 84.81 & 89.39 & 83.33 & 89.68 & \cellcolor{gray!20}{\textbf{90.15}} & 81.43 & 91.34 & \cellcolor{gray!20}{\textbf{91.77}} \\
        Worst     & 56.52 & 70.51 & 76.92 & 62.58 & 79.21 & \cellcolor{gray!20}{\textbf{81.34}} & 58.31 & 82.51 & \cellcolor{gray!20}{\textbf{84.20}} \\
	\bottomrule
\end{tabular}
\end{center}
\label{tab:cifar10n}
\vspace{-10pt}
\end{table*}
